On the second moment of the determinant of random symmetric, Wigner, and Hermitian matrices

In this paper, we analyze the second moment of the determinant of random symmetric, Wigner, and Hermitian matrices. Using analytic combinatorics techniques, we determine the second moment of the determinant of Hermitian matrices whose entries on the diagonal are i.i.d and whose entries above the diagonal are i.i.d. and have real expected values. Our results extend previous work analyzing the second moment of the determinant of symmetric and Wigner matrices, providing a unified approach for this analysis.

==> paraloops.tex <==
For each of the $(l-1)!$ parallel loops, we can think it as path of length $l$ which starts with $1$. Inside this loop, each consecutive pair that is increasing contributes $\lambda_{20}$ and each decreasing pair contributes $\overline{\lambda}_{20}$. The two edges connecting with $1$ always contribute $\lambda_{20}\overline{\lambda}_{20}$. So we just need to consider the remaining $l-1$ elements, which form a permutation of $l-1$ elements. Then counting the number of $l-1$ permutations that has $k$ increasing pairs can be done by using the eulerian number.
\begin{equation*}
K(l)=
\begin{cases}
\kappa_2& l\leq 1\\
\lambda_{22}& l= 2\\
\lambda_{11}^l(l-1)!+\sum^{l-2}_{k=0}A(l-1,k)\lambda_{20}^{k+1} \bar{\lambda}_{20}^{l-k-1}& l\geq 3, l $\text{ odd}$\\
2\lambda_{11}^{l}(l-1)!+\sum^{l-2}_{k=0}A(l-1,k)\lambda_{20}^{k+1} \bar{\lambda}_{20}^{l-k-1} & l\geq 4, l $\text{ even}$
\end{cases}
\end{equation*}
Where $A(n,k)=\sum^n_{i=0} (-1)^i \binom{n+1}{i}(k+1-i)^n$, which is the explicit formula for eularian numbers.

The Eulerian polynomials are defined by the exponential generating function 
$$\sum^{\infty}_{n=0}A_n(t)\frac{x^n}{n!}=\frac{t-1}{t-e^{(t-1)x}}.$$

The Eulerian numbers may be defined as the coefficients of the Eulerian polynomials:
$$A_n(t)=\sum^n_{k=0}A(n,k)t^k.$$

As before, we just need to sum all the terms to get the expression.
$$f^{sym}_2(n)=\sum^{n}_{i=1}\binom{n-1}{i-1}K(i)f^{sym}_2(n-i)$$ 
